How to reduce the search space of Entity Resolution: with Blocking or Nearest Neighbor search?

Entity Resolution suffers from quadratic time complexity. To increase its time efficiency, three kinds of filtering techniques are typically used for restricting its search space: (i) blocking workflows, which group together entity profiles with identical or similar signatures, (ii) string similarity join algorithms, which quickly detect entities more similar than a threshold, and (iii) nearest-neighbor methods, which convert every entity profile into a vector and quickly detect the closest entities according to the specified distance function. Numerous methods have been proposed for each type, but the literature lacks a comparative analysis of their relative performance. As we show in this work, this is a non-trivial task, due to the significant impact of configuration parameters on the performance of each filtering technique. We perform the first systematic experimental study that investigates the relative performance of the main methods per type over 10 real-world datasets. For each method, we consider a plethora of parameter configurations, optimizing it with respect to recall and precision. For each dataset, we consider both schema-agnostic and schema-based settings. The experimental results provide novel insights into the effectiveness and time efficiency of the considered techniques, demonstrating the superiority of blocking workflows and string similarity joins.

==> figures.tex <==
\begin{figure*}[ht!]
\centering
\includegraphics[width=0.99\textwidth]{figures/blockBuilding/saPC.png}
\includegraphics[width=0.99\textwidth]{figures/blockBuilding/saComp.png}
% \includegraphics[width=0.99\textwidth]{figures/blockBuilding/saRT.png}
\vspace{-14pt}
\caption{Performance of the schema-agnostic block building methods with respect to (i) $PC$ and (ii) $||B||$..}
\vspace{-10pt}
\label{fig:saBlockBuilding}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=0.99\textwidth]{figures/blockBuilding/sbBBpc.png}
\includegraphics[width=0.99\textwidth]{figures/blockBuilding/sbBBcomp.png}
% \includegraphics[width=0.99\textwidth]{figures/blockBuilding/sbBBrt.png}
\vspace{-14pt}
\caption{Performance of the schema-based block building methods with respect to (i) $PC$, a(ii) $||B||$ and (iii) $RT$.}
\vspace{-10pt}
\label{fig:sbBlockBuilding}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=0.99\textwidth]{figures/blockProcessing/saBPpc.png}
\includegraphics[width=0.99\textwidth]{figures/blockProcessing/saBPcomp.png}
% \includegraphics[width=0.99\textwidth]{figures/blockProcessing/saBPrt.png}
\vspace{-14pt}
\caption{Performance of the schema-agnostic block processing methods with respect to (i) $PC$ and (ii) $||B||$..}
\vspace{-10pt}
\label{fig:sBblockProcessing}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=0.99\textwidth]{figures/blockProcessing/sbBPpc.png}
\includegraphics[width=0.99\textwidth]{figures/blockProcessing/sbBPcomp.png}
% \includegraphics[width=0.99\textwidth]{figures/blockProcessing/sbBPrt.png}
\vspace{-14pt}
\caption{Performance of the schema-based block processing methods with respect to (i) $PC$ and (ii) $||B||$..}
\vspace{-10pt}
\label{fig:sBblockProcessing}
\end{figure*}

\begin{figure}[ht!]
\centering
\includegraphics[width=0.4\textwidth]{figures/simJoins/saPCJoin.png}
\includegraphics[width=0.4\textwidth]{figures/simJoins/saBJoin.png}
% \includegraphics[width=0.4\textwidth]{figures/simJoins/saRTJoin.png}
\vspace{-14pt}
\caption{Performance of the schema-agnostic similarity join methods with respect to (i) $PC$ and (ii) $||B||$..}
\vspace{-10pt}
\label{fig:saSimJoins}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[width=0.4\textwidth]{figures/simJoins/sbPCJoin.png}
\includegraphics[width=0.4\textwidth]{figures/simJoins/sbBJoin.png}
% \includegraphics[width=0.4\textwidth]{figures/simJoins/sbRTJoin.png}
\vspace{-14pt}
\caption{Performance of the schema-based similarity join methods with respect to (i) $PC$ and (ii) $||B||$..}
\vspace{-10pt}
\label{fig:sbSimJoins}
\end{figure}

==> tables/allResults.tex <==
\begin{table*}[t]\centering
\footnotesize
  \setlength{\tabcolsep}{3pt}
    \caption{The performance of the {\color{blue}blocking workflows}, {\color{teal}similarity join} and {\color{red}NN} methods across all datasets with respect to the number of candidates ($|C|$), recall ($PC$), precision ($PQ$) and the overall run-time ($RT$) in milliseconds ($ms$) or seconds ($s$).}
    \vspace{-10pt}
    \begin{tabular}{ | c l | r  r  r  r  r  r  r  r  r  r || r  r  r  r  r  r  |}
		\cline{3-18}
		\multicolumn{2}{c|}{} &
		\multicolumn{10}{c||}{\textbf{Schema-agnostic}}&
		\multicolumn{6}{c|}{\textbf{Schema-based}}\\
		\multicolumn{2}{c|}{} &
		\multicolumn{1}{c}{$\mathbf{D_{a1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a4}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a5}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a6}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a7}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a8}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a9}}$} &
        \multicolumn{1}{c||}{$\mathbf{D_{a10}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b4}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b8}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{b9}}$} \\
		\hline
        \hline
        \multirow{4}{*}{{\color{blue}\shortstack[c]{Standard\\ Blocking\\ (SBW)}}} & $|C|$ & 167 & 4,493 & 59,685 & 2,100 & 4,750 & 5,238 & 6,453 & 6,596 & 4,492 & 43,444 & 108 & 3,739 & 4,832 & 2,639 & 27,707 & 3,992 \\
        & $PC$ & 1.000 & 0.902 & 0.901 & 0.903 & 0.922 & 0.924 & 0.909 & 0.904 & 0.915 & 0.904 & 0.933 & 0.901 & 0.922 & 0.976 & 0.904 & 0.906 \\
        & $PQ$ & 0.533 & 0.216 & \underline{0.017} & \textbf{\underline{0.957}} & \textbf{\underline{0.382}} & \textbf{\underline{0.189}} & \underline{0.154} & \underline{0.117} & \underline{0.470} & \textbf{\underline{0.475}} & \textbf{\underline{0.769}} & 0.259 & 0.211 & 0.822 & 0.028 & \underline{0.524} \\
        & $RT$ & 27 ms & 225 ms & 359 ms & 58 ms & 316 ms & 1.1 s & 252 ms & 741 ms & 3.5 s & 57.7 s & 36 ms & 113 ms & 127 ms & 64 ms & 2.7 s & 4.0 s \\
		\hline
		\hline
		\multirow{4}{*}{{\color{blue}\shortstack[c]{Q-Grams\\ Blocking\\ (QBW)}}} & $|C|$ & 187 & 1,326 & 78,072 & 2,268 & 8,518 & 12,569 & 8,868 & 6,660 & 9,038 & 	59,275 & 110 & 1,312 & 4,217 & 2,704 & 25,819 & 9,231 \\
        & $PC$ & 0.978 & 0.912 & 0.902 & 0.915 & 0.910 & 0.910 & 0.903 & 0.904 & 0.993 & 0.900 & 0.933 & 0.914 & 0.915 & 0.952 & 0.903 & 0.928 \\
        & $PQ$ & 0.465 & 0.740 & 0.013 & 0.897 & 0.210 & 0.078 & 0.112 & 0.116 & 0.254	 & 0.347 & 0.755 & 0.750 & \textbf{\underline{0.240}} & 0.783 & \underline{0.030} & 0.232 \\
        & $RT$ & 46 ms & 75 ms & 340 ms & 92 ms & 234 ms & 1.2 s & 273 ms & 787 ms & 70.0 s & 158.6 s & 21 ms & 38 ms & 237 ms & 45 ms & 6.0 s & 3.6 s \\
        \hline 
        \hline
        {\color{blue}Extended} & $|C|$ & 107 & 4,746 & 81,496 & 2,205 & 8,084 & 12,459 & 7,976 & 8,869 & 14,164 & 52,739 & 110 & 3,719 & 5,307 & 2,377 & 36,076 & 11,530 \\
        {\color{blue}Q-Grams} & $PC$ & 0.910 & 0.901 & 0.905 & 0.918 & 0.905 & 0.904 & 0.905 & 0.900 & 0.913 & 0.900 & 0.944 & 0.902 & 0.905 & 0.913 & 0.903 & 0.910 \\
        {\color{blue}Blocking} & $PQ$ & 0.757 & 0.204 & 0.012 & 0.926 & 0.220 & 0.078 & 0.124 & 0.087 & 0.149 & 0.390 & 0.764 & 0.261 & 0.188 & \underline{0.854} & 0.021 & 0.182 \\
        {\color{blue}(EQBW)} & $RT$ & 303 ms & 347 ms & 2.2 s & 2.6 s & 411 ms & 603 ms & 704 ms & 1.2 s & 6.9 s & 68.1 s & 37 ms	 & 198 ms & 251 ms & 738 ms & 3.9 s & 5.0 s \\
        \hline 
        \hline
        {\color{blue}Suffix} & $|C|$ & 116 & 2,529 & 68,021 & 2,682 & 8,164 & 15,001 & 6,751 & 8,141 & 6,474 & 	1.0$\cdot$10$^6$ & 107 & 2,491 & 4,437 & 3,192 & 79,778 & 1.5$\cdot$10$^5$ \\
        {\color{blue}Arrays} & $PC$ & 1.000 & 0.901 & 0.900 & 0.969 & 0.900 & 0.903 & 0.901 & 0.912 & 0.902 & 0.900 & 0.910 & 0.903 & 0.909 & 0.997 & 0.900 & 0.877 \\
        {\color{blue}Blocking} & $PQ$ & \textbf{\underline{0.767}} & 0.384 & 0.015 & 0.804 & 0.217 & 0.065 & 0.146 & 0.096 & 0.322 & 	0.020 & 0.757 & 0.390 & 0.226 & 0.695 & 0.010 & 0.014 \\
        {\color{blue}(SABW)} & $RT$ & 49 ms & 142 ms & 676 ms & 238 ms & 305 ms & 347 ms & 436 ms & 674 ms & 3.0 s & 9.8 s & 19 ms & 58 ms & 114 ms & 337 ms & 645 ms & 4.5 s \\
        \hline 
        \hline
        {\color{blue}Extended} & $|C|$ & 175 & 1,277 & 96,064 & 2,674 & 8,819 & 16,473 & 7,261 & 8,705 & 16,016	& 1.5$\cdot$10$^6$ & 109 & 1,243 & 7,567 & 3,683 & 88,236 & 2.0$\cdot$10$^5$ \\
        {\color{blue}Suffix Arrays}& $PC$ & 0.921 & 0.901 & 0.902 & 0.902 & 0.900 & 0.900 & 0.901 & 0.900 & 0.900 & 0.901 & 0.910 & 0.901 & 0.901 & 0.902 & 0.900 & 0.865 \\
        {\color{blue}Blocking} & $PQ$ & 0.469 & \textbf{\underline{0.759}} & 0.010 & 0.751 & 0.201 & 0.059 & 0.136 & 0.088 & 0.130	 & 0.014 & 0.743 & \textbf{\underline{0.780}} & 0.131 & 0.545 & 0.009 & 0.010 \\
        {\color{blue}(ESABW)} & $RT$ & 161 ms & 281 ms & 891 ms & 745 ms & 388 ms & 481 ms & 750 ms & 1.2 s & 5.6 s & 13.3 s & 23 ms & 187 ms & 418 ms & 201 ms & 1.3 s & 2.2 s \\
        \hline 
        \hline
        \multirow{4}{*}{{\color{blue}\shortstack[c]{Parameter-\\ free BW}}} & $|C|$ & 290 & 69,340 & 4.6$\cdot$10$^5$ & 1.1$\cdot$10$^5$ & 3.2$\cdot$10$^5$ & 2.6$\cdot$10$^5$ & 4.2$\cdot$10$^5$ & 1.9$\cdot$10$^6$ & 2.3$\cdot$10$^6$ & 6.9$\cdot$10$^7$ & 210 & 6,571 & 6,885 & 2,290 & 38,630 & 3,111 \\
        & $PC$ & 1.000 & 0.981 & 0.971 & 0.999 & 0.998 & 0.995 & 0.991 & 1.000 & 1.000 & 0.980 & 
        0.989 & 0.746 & 0.936 & 0.838 & 0.996 & 0.935 \\
        & $PQ$ & 0.307 & 0.015 & 0.002 & 0.020 & 0.006 & 0.004 & 0.003 & 4.5$\cdot$10$^{-4}$ & 0.001 & 3.3$\cdot$10$^{-4}$ & 0.162 & 0.175 & 0.047 & 0.230 & 5.8$\cdot$10$^{-4}$ & 0.005 \\
        & $RT$ & 29 ms & 32 ms & 135 ms & 44 ms & 76 ms & 81 ms & 125 ms & 243 ms & 579 ms & 5.1 s & 20 ms & 14 ms & 24 ms & 21 ms & 164 ms & 255 ms \\
        \hline
        \hline
        \multirow{4}{*}{{\color{blue}\shortstack[f]{Default\\ BW}}} & $|C|$ & 3.3$\cdot$10$^5$ & 15,350 & 2.0$\cdot$10$^5$ & 53,203 & 51,573 & 1.2$\cdot$10$^5$ & 1.3$\cdot$10$^5$ & 4.1$\cdot$10$^5$ & 8.4$\cdot$10$^5$ & 2.4$\cdot$10$^6$ & 272 & 5,859 & 14,302 & 35,114 & 1.6$\cdot$10$^5$ & 7.0$\cdot$10$^5$ \\
        & $PC$ & 1.000 & 0.930 & 0.936 & 1.000 & 0.943 & 0.894 & 0.984 & 0.996 & 0.997 & 0.922 & 	0.607 & 0.888 & 0.894 & 0.999 & 0.931 & 0.995 \\
        & $PQ$ & 2.7$\cdot$10$^{-4}$ & 0.065 & 0.005 & 0.042 & 0.036 & 0.008 & 0.008 & 0.002 & 0.003 & 0.009 & 0.199 & 0.163 & 0.069 & 0.063 & 0.005 & 0.003 \\
        & $RT$ & 209 ms & 55 ms & 435 ms & 153 ms & 252 ms & 368 ms & 526 ms & 1.0 s & 2.5 s & 8.2 s & 17 ms & 35 ms & 111 ms & 76 ms & 637 ms & 1.7 s \\
        \hline
        \hline
        \multirow{4}{*}{{\color{teal}$\epsilon$-Join}} & $|C|$ & 112 & 10,194 & 1.02$\cdot$10$^5$ & 2,120 & 98,786 & 6.8$\cdot$10$^5$ & 5,132 & 11,332 & 2,719 & 6.2$\cdot$10$^5$ & 210 & 6,571 & 6,885 & 2,290 & 38,630 & 3,111 \\
        & $PC$ & 0.921 & 0.903 & 0.911 & 0.901 & 0.911 & 0.901 & 0.900 & 0.902 & 0.901 & 0.902 & 0.900	& 0.901 & 0.900 & 0.913 & 0.907 & 0.901 \\
        & $PQ$ & \underline{0.732} & 0.095 & 0.010 & 0.945 & 0.018 & 0.001 & \textbf{\underline{0.192}} & 0.068 & 0.765 & 0.033 & \underline{0.381} & 0.147 & 0.144 & \underline{0.886} & 0.020 & \underline{0.669} \\
        & $RT$ & 278 ms & 703 ms & 811 ms & 575 ms & 2.8 s & 8.8 s & 2.8 s & 15.1 s & 30.9 s & 39.4 s & 128 ms & 418 ms & 235 ms & 163 ms & 8.2 s & 24.6 s \\
        \hline
        \hline
        \multirow{4}{*}{{\color{teal}kNN-Join}} & $|C|$ & 398 & 4,345 & 35,333 & 2,323 & 6,195 & 8,013 & 8,194 & 5,163 & 2,520 & 1.4$\cdot$10$^5$ & 282 & 3,375 & 4,210 & 2,642 & 15,581 & 3,462 \\
        & $PC$ & 1.000 & 0.924 & 0.900 & 0.996 & 0.961 & 0.910 & 0.972 & 0.910 & 0.957 & 0.903 & 0.978 & 0.925 & 0.914 & 0.994 & 0.900 & 0.970  \\
        & $PQ$ & 0.224 & \underline{0.229} & \textbf{\underline{0.028}} & \underline{0.954} & \underline{0.305} & \underline{0.122} & 0.130 & \textbf{\underline{0.150}} & \textbf{\underline{0.877}} & \underline{0.149} & 0.309 & \underline{0.295} & \textbf{\underline{0.240}} & 0.836 & \textbf{\underline{0.049}} & 0.647 \\
        & $RT$ & 1.1 s & 874 ms & 4.5 s & 4.4 s & 1.8 s & 1.2 s & 1.8 s & 12.2 s & 26.2 s & 93.9 s & 130 ms & 490 ms & 660 ms & 921 ms & 15.0 s & 47.6 s \\
        \hline
        \hline
        & $|C|$ & 1,909 & 5,451 & 6,844 & 11,649 & 32,920 & 41,450 & 41,034 & 12,884 & 12,638 & 1.3$\cdot$10$^5$ & 870 & 5,686 & 6,909 & 11,929 & 13,277 & 13,593 \\
        {\color{teal}Default} & $PC$ & 1.000 & 0.915 & 0.804 & 0.998 & 0.882 & 0.921 & 0.984 & 0.939 & 0.995 & 0.887 & 1.000 & 0.916 & 0.934 & 0.998 & 0.831 & 0.989 \\
        {\color{teal}kNN-Join} & $PQ$ & 0.047 & 0.181 & 0.130 & 0.190 & 0.053 & 0.024 & 0.026 & 0.062 & 0.182 & 0.147 & 0.100 & 0.173 & 0.149 & 0.187 & 0.054 & 0.166\\
        & $RT$ & 969 ms & 750 ms & 4.4 s & 2.0 s & 3.6 s & 3.0 s & 3.6 s & 10.7 s & 24.1 & 91.3 s & 
        133 ms & 312 ms & 677 ms & 883 ms & 5.1 s & 12.0 s \\
        \hline
        \hline
        & $|C|$ & 3.8$\cdot$10$^5$ & 1.1$\cdot$10$^6$ & 3.7$\cdot$10$^6$ & 3.9$\cdot$10$^5$ & 2.7$\cdot$10$^7$ & 3.9$\cdot$10$^7$ & 3.1$\cdot$10$^7$ & 4.9$\cdot$10$^7$ & 1.0$\cdot$10$^8$ & - & 11,411 & 1.0$\cdot$10$^6$ & 3.6$\cdot$10$^6$ & 64,398 & 4.9$\cdot$10$^6$ & - \\
        {\color{red}MinHash} & $PC$ & 0.910 & 0.987 & 0.903 & 0.903 & 0.903 & 0.985 & 0.936 & 0.948 & 0.923 & - & 0.900 & 0.942 & 0.936 & 0.973 & 0.955 & - \\
        {\color{red}LSH} & $PQ$ & 2.6$\cdot$10$^{-4}$ & 0.001 & 2.7$\cdot$10$^{-4}$ & 0.005 & 6.6$\cdot$10$^{-5}$ & 2.7$\cdot$10$^{-5}$ & 3.4$\cdot$10$^{-5}$ & 1.6$\cdot$10$^{-5}$ & 2.1$\cdot$10$^{-5}$ & - & 0.007 & 0.001 & 2.9$\cdot$10$^{-4}$ & 0.036 & 1.7$\cdot$10$^{-5}$ & -\\
        & $RT$ & 212 ms & 717 ms & 4.3 s & 365 ms & 10.3 s & 38.8 s & 12.9 s & 18.3 s & 29.4 s & - & 153 ms & 598 ms & 1.2 s & 2.8 s & 18.8 s & -\\
        \hline
        \hline
        \multirow{4}{*}{\color{red}{\shortstack[c]{Cross-\\ Polytope\\LSH}}} & $|C|$ & 23,590 & 1.6$\cdot$10$^5$ & 1.2$\cdot$10$^6$ & 25,344 & 3.2$\cdot$10$^6$ & 4.7$\cdot$10$^6$ & 5.7$\cdot$10$^5$ & 1.9$\cdot$10$^6$ & 9.6$\cdot$10$^6$ & 2.6$\cdot$10$^8$ & 622 & 1.3$\cdot$10$^5$ & 3.5$\cdot$10$^5$ & 2,286	 & 6.9$\cdot$10$^5$ & 1.3$\cdot$10$^6$ \\
        & $PC$ & 0.910 & 0.908 & 0.900 & 0.900 & 0.901 & 0.905 & 0.900 & 0.900 & 0.901 & 0.901 & 	0.910 & 0.911 & 0.902 & 0.901 & 0.917 & 0.908 \\
        & $PQ$ & 0.003 & 0.006 & 0.001 & 0.079 & 0.001 & 2.1$\cdot$10$^{-4}$ & 0.002 & 4.0$\cdot$10$^{-4}$ & 2.2$\cdot$10$^{-4}$	& 7.8$\cdot$10$^{-5}$ & 0.130 & 0.008 & 0.003 & 0.876 & 0.001 & 0.002 \\
        & $RT$ & 181 ms & 902 ms & 4.3 s & 2.0 s & 1.7 s & 1.8 s & 3.6 s & 4.8 s & 19.9 s & 63.9 s & 208 ms & 420 ms & 927 ms & 646 ms & 7.5 s & 7.4 s \\
	    \hline
        \hline
        & $|C|$ & 34,118 & 2.4$\cdot$10$^5$ & 1.8$\cdot$10$^6$ & 34,148 & 4.1$\cdot$10$^6$ & 4.6$\cdot$10$^6$ & 6.7$\cdot$10$^5$ & 3.0$\cdot$10$^6$ & 1.4$\cdot$10$^7$ & 2.8$\cdot$10$^8$ & 1,328 & 1.3$\cdot$10$^5$ & 6.4$\cdot$10$^5$ & 2,375 & 1.9$\cdot$10$^6$ & 87,651 \\
        {\color{red}Hyper-} & $PC$ & 0.910 & 0.901 & 0.900 & 0.900 & 0.900 & 0.900 & 0.900 & 0.900 &  
        0.900 & 0.900 & 0.910 & 0.900 & 0.900 & 0.917 & 0.900 & 0.900 \\
        {\color{red}plane LSH} & $PQ$ & 0.002 & 0.004 & 0.001 & 0.059 & 4.4$\cdot$10$^{-4}$ & 2.1$\cdot$10$^{-4}$ & 0.001 & 2.6$\cdot$10$^{-4}$ & 1.5$\cdot$10$^{-4}$ & 7.3$\cdot$10$^{-5}$ & 0.061 & 0.007 & 0.002 & 0.859 & 4.0$\cdot$10$^{-4}$ & 0.024 \\
        & $RT$ & 168 ms & 940 ms & 4.2 s & 1.9 s & 1.6 s & 3.5 s & 4.4 s & 7.5 s & 17.5 s & 71.1 s & 246 ms & 430 ms & 930 ms & 943 ms & 5.2 s & 7.0 s \\
        \hline
        \hline
        \multirow{4}{*}{{\color{red}FAISS}} & $|C|$ & 1,017 & 30,128 & 1.7$\cdot$10$^6$ & 2,294 & 1.5$\cdot$10$^5$ & 2.0$\cdot$10$^5$ & 24,224 & 5.3$\cdot$10$^5$ & 1.8$\cdot$10$^5$ & 1.3$\cdot$10$^8$8 & 226 & 19,368 & 41,974 & 2,293 & 2.0$\cdot$10$^5$ & 2,516 \\
        & $PC$ & 0.933 & 0.902 & 0.900 & 0.961 & 0.901 & 0.900 & 0.908 & 0.900 & 0.900 & 0.900 & 0.955 & 0.906 & 0.900 & 0.971 & 0.900 & 0.912 \\
        & $PQ$ & 0.082 & \underline{0.032} & 0.001 & 0.932 & \underline{0.012} & \underline{0.005} & 0.041 & 0.001 & 0.012 & 1.5$\cdot$10$^{-4}$ & 0.376 & \underline{0.050} & 0.024 & \textbf{\underline{0.942}} & 0.004 & \textbf{\underline{0.836}} \\
        & $RT$ & 164 ms & 790 ms & 4.2 s & 1.5 s & 1.4 s & 1.8 s & 2.1 s & 7.5 s & 17.7 s & 53.3 s & 204 ms & 264 ms & 787 ms & 901 ms & 5.1 s & 7.4 s \\
        \hline
        \hline
        \multirow{4}{*}{{\color{red}SCANN}} & $|C|$ & 1,017 & 30,128 & 1.4$\cdot$10$^6$ & 2,294 & 1.5$\cdot$10$^5$ & 2.0$\cdot$10$^5$ & 24,224 & 4.2$\cdot$10$^5$ & 1.6$\cdot$10$^6$ & 1.3$\cdot$10$^8$ & 226 & 19,368 & 41,974 & 2,293 & 1.5$\cdot$10$^5$ & 2,516 \\
        & $PC$ & 0.933 & 0.902 & 0.900 & 0.961 & 0.901 & 0.900 & 0.908 & 0.900 & 0.900 & 0.900 & 0.966 & 0.906 & 0.900 & 0.970 & 0.900 & 0.912 \\
        & $PQ$ & 0.082 & \underline{0.032} & 0.001 & 0.932 & \underline{0.012} & \underline{0.005} & 0.041 & 0.002 & 0.013 & 1.5$\cdot$10$^{-4}$ & \underline{0.381} & \underline{0.050} & 0.024 & 0.941 & 0.005 & \textbf{\underline{0.836}} \\
        & $RT$ & 182 ms & 828 ms & 4.6 s & 1.8 s & 2.1 s & 2.5 s & 3.0 s & 9.5 s & 29.5 s & 74.4 s & 741 ms & 319	ms & 841 ms & 1.1 s & 9.4 s & 7.8 s \\
        \hline
        \hline
        & $|C|$ & 339 & 37,660 & 5.5$\cdot$10$^5$ & 2,294 & 1.6$\cdot$10$^5$ & 3.2$\cdot$10$^5$ & 7,810 & 43,418 & 12,580 & -
        & 339 & 33,356 & 13,540 & 2,294 & 63,850 & 10,064 \\
        {\color{red}Deep-} & $PC$ & 0.943 & 0.903 & 0.900 & 0.983 & 0.901 & 0.900 & 0.926 & 0.900 & 0.908 & - & 0.976 & 0.900 & 0.900 & 0.964 & 0.900 & 0.919 \\
        {\color{red}Blocker} & $PQ$ & \underline{0.247} & 0.026 & \underline{0.002} & \underline{0.953} & 0.011 & 0.004 & \underline{0.130} & \underline{0.018} & \underline{0.167} & - & 0.256 & 0.029 & \underline{0.073} & 0.935 & \underline{0.012} & 0.211 \\
        & $RT$ & 6.7 s & 7.5 s & 26.2 s & 18.7 s & 41.4 s & 43.1 s & 46.9 s & 91.1 s & 241.5 s & - & 5.8  s & 5.6	s & 12.2 s & 11.9 s & 89.2 s & 199.8 s \\
        \hline
        \hline
        \multirow{4}{*}{\color{red}{\shortstack[c]{Defalut\\ Deep-\\Blocker}}}& $|C|$ & 11,280 & 5,380 & 15,195 & 13,080 & 30,280 & 39,050 & 39,050 & 1.1$\cdot$10$^5$ & 3.1$\cdot$10$^6$ & - & 11,280 & 5,380 & 15,195 & 13,080 & 1.1$\cdot$10$^5$ & 3.1$\cdot$10$^6$ \\
        & $PC$ & 0.970 & 0.732 & 0.652 & 0.996 & 0.822 & 0.745 & 0.949 & 0.938 & 0.966 & -  & 0.992 & 0.800 & 0.839 & 0.990 & 0.900 & 0.972\\
        & $PQ$ & 0.008 & 0.146 & 0.047 & 0.169 & 0.053 & 0.020 & 0.027 & 0.007 & 0.007 & - & 0.008 & 0.160 & 0.061 & 0.168 & 0.007 & 0.007 \\
        & $RT$ & 6.5 s & 6.6 s & 20.0 s & 15.8 s & 39.4 s & 42.2 s & 44.8 s & 83.2 s & 206.5 s & - & 4.9 s & 5.0 s & 11.1 s & 13.0 s & 79.9 s & 185.9 s \\
        \hline
	\end{tabular}
	\label{tb:blockingPerformance}
	\vspace{-10pt}
\end{table*}

==> tables/blockBuildingConfiguration.tex <==
\begin{table*}[t]\centering
\small
% \setlength{\tabcolsep}{4.5pt}
    \caption{The best configuration of each block building method across all datasets, both in schema-agnostic and schema-based settings. Token Blocking is excluded, as it is a parameter-free approach.}
    \vspace{-10pt}
	\begin{tabular}{ | l | l | r | r | r | r | r | r | r | r | r | r || r | r | r | r | r | r | r | r | r | r |}
		\cline{3-22}
		\multicolumn{2}{c|}{} &
		\multicolumn{10}{c||}{\textbf{Schema-agnostic}}&
		\multicolumn{10}{c|}{\textbf{Schema-based}}\\
		\multicolumn{2}{c|}{} &
		\multicolumn{1}{c|}{$\mathbf{D_{c1}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c2}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c3}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c4}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c5}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c6}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c7}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c8}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c9}}$} &
        \multicolumn{1}{c||}{$\mathbf{D_{c10}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c1}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c2}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c3}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c4}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c5}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c6}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c7}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c8}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c9}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c10}}$}\\
		\hline
        \hline
        \textsf{SN} & $w$ & 2 & 4 & 7 & 2 & 5 & 7 & 4 & 4 & 8 & 17 & 2 & 5 & 7 & 5 & 65 & 33 & 90 & 16 & 25 & 100 \\
        \hline
        \textsf{QB} & $q$ & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 2 & 2 & 2 & 6 & 6 & 2 \\
        \hline
        \multirow{ 2}{*}{\textsf{EQB}} & $q$ & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 2 & 2 & 2 & 6 & 6 & 2 \\
        & $t$ & 0.9 & 0.9 & 0.9 & 0.9 & 0.9 & 0.9 & 0.9 & 0.9 & 0.9 & 0.9 & 0.9 & 0.9 & 0.9 & 0.9 & 0.8 & 0.8 & 0.8 & 0.9 & 0.9 & 0.8 \\
        \hline
        \multirow{ 2}{*}{\textsf{SA}} & $l_{min}$ & 6 & 3 & 6 & 6 & 6 & 6 & 6 & 4 & 6 & 6 & 6 & 5 & 6 & 6 & 2 & 2 & 2 & 6 & 6 & 5 \\
        & $b_{max}$ & 2 & 16 & 37 & 8 & 15 & 21 & 13 & 13 & 34 & 76 & 4 & 26 & 22 & 18 & 33 & 90 & 90 & 77 & 100 & 100 \\
        \hline
        \multirow{ 2}{*}{\textsf{ESA}} & $l_{min}$ & 6 & 4 & 6 & 6 & 6 & 6 & 6 & 5 & 6 & 6 & 6 & 4 & 6 & 6 & 2 & 2 & 2 & 6 & 6 & 5 \\
        & $b_{max}$ & 3 & 7 & 39 & 8 & 16 & 21 & 13 & 10 & 35 & 77 & 4 & 8 & 22 & 19 & 37 & 91 & 90 & 78 & 100 & 100 \\
		\hline
	\end{tabular}
	\label{tb:ccerDatasets}
\end{table*}

==> tables/candidates.tex <==
\begin{table*}[b]\centering
\scriptsize
  \setlength{\tabcolsep}{2.2pt}
    \caption{The number of candidate pairs per method, dataset and schema settings.}
    \vspace{-8pt}
    \begin{tabular}{ | l | r  r  r  r  r  r  r  r  r  r || r  r  r  r  r  r  |}
		\cline{2-17}
		\multicolumn{1}{c|}{} &
		\multicolumn{10}{c||}{\textbf{Schema-agnostic Settings}}&
		\multicolumn{6}{c|}{\textbf{Schema-based Settings}}\\
		\multicolumn{1}{c|}{} &
		\multicolumn{1}{c}{$\mathbf{D_{a1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a4}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a5}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a6}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a7}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a8}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a9}}$} &
        \multicolumn{1}{c||}{$\mathbf{D_{a10}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b4}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b8}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{b9}}$} \\
		\hline
        \hline
        SBW & 167 & 4,493 & \underline{59,685} & \textbf{\underline{2,100}} & \textbf{\underline{4,750}} & \textbf{\underline{5,238}} & \underline{6,453} & \underline{6,596} & \underline{4,492} & \textbf{\underline{43,444}} & \textbf{\underline{108}} & 3,739 & 4,832 & 2,639 & 27,707 & \underline{3,992} \\
        QBW & 187 & 1,326 & 78,072 & 2,268 & 8,518 & 12,569 & 8,868 & 6,660 & 9,038 & 59,275 & 110 & 1,312 & \textbf{\underline{4,217}} & 2,704 & \underline{25,819} & 9,231 \\
        EQBW & 107 & 4,746 & 81,496 & 2,205 & 8,084 & 12,459 & 7,976 & 8,869 & 14,164 & 52,739 & 110 & 3,719 & 5,307 & \underline{2,377} & 36,076 & 11,530 \\
        SABW & \textbf{\underline{116}} & 2,529 & 68,021 & 2,682 & 8,164 & 15,001 & 6,751 & 8,141 & 6,474 & 	1.0$\cdot$10$^6$ & 107 & 2,491 & 4,437 & 3,192 & 79,778 & 1.5$\cdot$10$^5$ \\
        ESABW & 175 & \textbf{\underline{1,277}} & 96,064 & 2,674 & 8,819 & 16,473 & 7,261 & 8,705 & 16,016	& 1.5$\cdot$10$^6$ & 109 & \textbf{\underline{1,243}} & 7,567 & 3,683 & 88,236 & 2.0$\cdot$10$^5$ \\
        PBW & 290 & 69,340 & 4.6$\cdot$10$^5$ & 1.1$\cdot$10$^5$ & 3.2$\cdot$10$^5$ & 2.6$\cdot$10$^5$ & 4.2$\cdot$10$^5$ & 1.9$\cdot$10$^6$ & 2.3$\cdot$10$^6$ & 6.9$\cdot$10$^7$ & 210 & {\color{red}6,571} & 6,885 & {\color{red}2,290} & 38,630 & 3,111 \\
        DBW & 3.3$\cdot$10$^5$ & 15,350 & 2.0$\cdot$10$^5$ & 53,203 & 51,573 & 1.2$\cdot$10$^5$ & 1.3$\cdot$10$^5$ & 4.1$\cdot$10$^5$ & 8.4$\cdot$10$^5$ & 2.4$\cdot$10$^6$ & {\color{red}272} & {\color{red}5,859} & 14,302 & 35,114 & 1.6$\cdot$10$^5$ & 7.0$\cdot$10$^5$ \\
        \hline
        \hline
        $\epsilon$-Join & \underline{112} & 10,194 & 1.02$\cdot$10$^5$ & 2,120 & 98,786 & 6.8$\cdot$10$^5$ & \textbf{\underline{5,132}} & 11,332 & 2,719 & 6.2$\cdot$10$^5$ & \underline{210} & 6,571 & 6,885 & \underline{2,290} & 38,630 & \underline{3,111} \\
        kNNj & 398 & \underline{4,345} & \textbf{\underline{35,333}} & \underline{2,323} & \underline{6,195} & \underline{8,013} & 8,194 & \textbf{\underline{5,163}} & \textbf{\underline{2,520}} & \underline{1.4$\cdot$10$^5$} & 282 & \underline{3,375} & \textbf{\underline{4,210}} & 2,642 & \textbf{\underline{15,581}} & 3,462 \\
        DkNN & 1,909 & 5,451 & {\color{red}6,844} & 11,649 & {\color{red}32,920} & 41,450 & 41,034 & 12,884 & 12,638 & {\color{red}1.3$\cdot$10$^5$} & 870 & 5,686 & 6,909 & 11,929 & {\color{red}13,277} & 13,593 \\
        \hline
        \hline
        MH-LSH & 3.8$\cdot$10$^5$ & 1.1$\cdot$10$^6$ & 3.7$\cdot$10$^6$ & 3.9$\cdot$10$^5$ & 2.7$\cdot$10$^7$ & 3.9$\cdot$10$^7$ & 3.1$\cdot$10$^7$ & 4.9$\cdot$10$^7$ & 1.0$\cdot$10$^8$ & - & 11,411 & 1.0$\cdot$10$^6$ & 3.6$\cdot$10$^6$ & 64,398 & 4.9$\cdot$10$^6$ & - \\
        CP-LSH & 23,590 & 1.6$\cdot$10$^5$ & 1.2$\cdot$10$^6$ & 25,344 & 3.2$\cdot$10$^6$ & 4.7$\cdot$10$^6$ & 5.7$\cdot$10$^5$ & 1.9$\cdot$10$^6$ & 9.6$\cdot$10$^6$ & 2.6$\cdot$10$^8$ & 622 & 1.3$\cdot$10$^5$ & 3.5$\cdot$10$^5$ & 2,286	 & 6.9$\cdot$10$^5$ & 1.3$\cdot$10$^6$ \\
        HP-LSH & 34,118 & 2.4$\cdot$10$^5$ & 1.8$\cdot$10$^6$ & 34,148 & 4.1$\cdot$10$^6$ & 4.6$\cdot$10$^6$ & 6.7$\cdot$10$^5$ & 3.0$\cdot$10$^6$ & 1.4$\cdot$10$^7$ & 2.8$\cdot$10$^8$ & 1,328 & 1.3$\cdot$10$^5$ & 6.4$\cdot$10$^5$ & 2,375 & 1.9$\cdot$10$^6$ & 87,651 \\
        FAISS & 1,017 & \underline{30,128} & 1.7$\cdot$10$^6$ & 2,294 & \underline{1.5$\cdot$10$^5$} & \underline{2.0$\cdot$10$^5$} & 24,224 & 5.3$\cdot$10$^5$ & 1.8$\cdot$10$^5$ & \underline{1.3$\cdot$10$^8$} & 226 & \underline{19,368} & 41,974 & \textbf{\underline{2,293}} & 2.0$\cdot$10$^5$ & \textbf{\underline{2,516}} \\
        SCANN & 1,017 & \underline{30,128} & 1.4$\cdot$10$^6$ & 2,294 & \underline{1.5$\cdot$10$^5$} & \underline{2.0$\cdot$10$^5$} & 24,224 & 4.2$\cdot$10$^5$ & 1.6$\cdot$10$^6$ & \underline{1.3$\cdot$10$^8$} & \underline{226} & \underline{19,368} & 41,974 & 2,293 & 1.5$\cdot$10$^5$ & \textbf{\underline{2,516}} \\
        DeepBlocker & \underline{339} & 37,660 & \underline{5.5$\cdot$10$^5$} & \underline{2,294} & 1.6$\cdot$10$^5$ & 3.2$\cdot$10$^5$ & \underline{7,810} & \underline{43,418} & \underline{12,580} & - & 339 & 33,356 & \underline{13,540} & 2,294 & \underline{63,850} & 10,064 \\
        DDB & 11,280 & {\color{red}5,380} & {\color{red}15,195} & 13,080 & {\color{red}30,280} & {\color{red}39,050} & 39,050 & 1.1$\cdot$10$^5$ & 3.1$\cdot$10$^6$ & - & 11,280 & {\color{red}5,380} & {\color{red}15,195} & 13,080 & 1.1$\cdot$10$^5$ & 3.1$\cdot$10$^6$ \\
        \hline
	\end{tabular}
	\label{tb:candidates}
	\vspace{-16pt}
\end{table*}

==> tables/joinsPerformance.tex <==
\begin{table*}[t]\centering
\footnotesize
\setlength{\tabcolsep}{4.5pt}
    \caption{The performance of the fine-tuned similarity join methods across all datasets with respect to number of candidates ($|C|$), recall ($PC$), precision ($PQ$) and overall run-time ($RT$), which is reported in milliseconds ($ms$) or seconds ($s$).}
    \vspace{-10pt}
    \begin{tabular}{ | c l | r  r  r  r  r  r  r  r  r  r || r  r  r  r  r  r  |}
		\cline{3-18}
		\multicolumn{2}{c|}{} &
		\multicolumn{10}{c||}{\textbf{Schema-agnostic}}&
		\multicolumn{6}{c|}{\textbf{Schema-based}}\\
		\multicolumn{2}{c|}{} &
		\multicolumn{1}{c}{$\mathbf{D_{a1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a4}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a5}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a6}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a7}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a8}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a9}}$} &
        \multicolumn{1}{c||}{$\mathbf{D_{a10}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b4}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b8}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{b9}}$} \\
		\hline
        \hline
        \multirow{4}{*}{$\epsilon$-Join} & $|C|$ & 112 & 10,194 & 1.02$\cdot$10$^5$ & 2,120 & 98,786 & 6.8$\cdot$10$^5$ & 5,132 & 11,332 & 2,719 & 6.2$\cdot$10$^5$ & 210 & 6,571 & 6,885 & 2,290 & 38,630 & 3,111 \\
        & $PC$ & 0.921 & 0.903 & 0.911 & 0.901 & 0.911 & 0.901 & 0.900 & 0.902 & 0.901 & 0.902 & 0.900	& 0.901 & 0.900 & 0.913 & 0.907 & 0.901 \\
        & $PQ$ & \underline{0.732} & 0.095 & 0.010 & 0.945 & 0.018 & 0.001 & \textbf{\underline{0.192}} & 0.068 & 0.765 & 0.033 & \underline{0.381} & 0.147 & 0.144 & \underline{0.886} & 0.020 & \underline{0.669} \\
        & $RT$ & 278 ms & 703 ms & 811 ms & 575 ms & 2.8 s & 8.8 s & 2.8 s & 15.1 s & 30.9 s & 39.4 s & 128 ms & 418 ms & 235 ms & 163 ms & 8.2 s & 24.6 s \\
        \hline
        % \multicolumn{21}{c}{\textbf{(b) kNN-Join}} \\
        \hline
        \multirow{4}{*}{kNN-Join} & $|C|$ & 398 & 4,345 & 35,333 & 2,323 & 6,195 & 8,013 & 8,194 & 5,163 & 2,520 & 1.4$\cdot$10$^5$ & 282 & 3,375 & 4,210 & 2,642 & 15,581 & 3,462 \\
        & $PC$ & 1.000 & 0.924 & 0.900 & 0.996 & 0.961 & 0.910 & 0.972 & 0.910 & 0.957 & 0.903 & 0.978 & 0.925 & 0.914 & 0.994 & 0.900 & 0.970  \\
        & $PQ$ & 0.224 & \underline{0.229} & \textbf{\underline{0.028}} & \underline{0.954} & \underline{0.305} & \underline{0.122} & 0.130 & \textbf{\underline{0.150}} & \textbf{\underline{0.877}} & \underline{0.149} & 0.309 & \underline{0.295} & \textbf{\underline{0.240}} & 0.836 & \textbf{\underline{0.049}} & 0.647 \\
        & $RT$ & 1.1 s  & 874 ms & 4.5 s & 4.4 s & 1.8 s & 1.2 s & 1.8 s & 12.2 s & 26.2 s & 93.9 s & 130 ms & 490 ms & 660 ms & 921 ms & 15.0 s & 47.6 s \\
        % \hline
        % % \multicolumn{21}{c}{\textbf{(c) Edit-based }} \\
        % \hline
        % & $|C|$ & - & - & - & - & - & - & - & - & - & - & 1,364 & 1,455 & 1,364 & 2,990 & 6,507 & 6,506\\
        % (c) Edit- & $PC$ & - & - & - & - & - & - & - & - & - & - & 0.011 & 0.359 & 0.295 & 0.978 & 0.382 & 0.933 \\
        % based Join & $PQ$ & - & - & - & - & - & - & - & - & - & - & 0.001 & 0.265 & 0.239 & 0.728 & 0.050 & 0.331 \\
        % & $RT$ &  - & - & - & - & - & - & - & - & - & - & 493 & 21.4 s & 67.0 s & \\
        \hline
        \hline
        & $|C|$ & 1,909 & 5,451 & 6,844 & 11,649 & 32,920 & 41,450 & 41,034 & 12,884 & 12,638 & 1.3$\cdot$10$^5$ & 870 & 5,686 & 6,909 & 11,929 & 13,277 & 13,593 \\
        Default & $PC$ & 1.000 & 0.915 & 0.804 & 0.998 & 0.882 & 0.921 & 0.984 & 0.939 & 0.995 & 0.822 & 1.000 & 0.914 & 0.928 & 0.998 & 0.822 & 0.987 \\
        kNN-Join & $PQ$ & 0.047 & 0.181 & 0.130 & 0.190 & 0.053 & 0.024 & 0.026 & 0.062 & 0.182 & 0.149 & 0.102 & 0.173 & 0.148 & 0.186 & 0.053 & 0.168\\
        & $RT$ & 969 ms & 750 ms & 4.4 s & 2.0 s & 3.6 s & 3.0 s & 3.6 s & 10.7 s & 24.1 & 91.3 s & 
        133 ms & 312 ms & 677 ms & 883 ms & 5.1 s & 12.0 s \\
        \hline
	\end{tabular}
	\label{tb:sjPerformance}
\end{table*}


==> tables/nnPerformance.tex <==
\begin{table*}[t]\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
    \caption{The performance of the fine-tuned vector-based NN methods across all datasets with respect to number of candidates ($|C|$), recall ($PC$), precision ($PQ$) and overall run-time ($RT$), which is reported in milliseconds ($ms$) or seconds ($s$).}
    \vspace{-10pt}
    \begin{tabular}{ | c l | r  r  r  r  r  r  r  r  r  r || r  r  r  r  r  r  |}
		\cline{3-18}
		\multicolumn{2}{c|}{} &
		\multicolumn{10}{c||}{\textbf{Schema-agnostic}}&
		\multicolumn{6}{c|}{\textbf{Schema-based}}\\
		\multicolumn{2}{c|}{} &
		\multicolumn{1}{c}{$\mathbf{D_{a1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a4}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a5}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a6}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a7}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a8}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a9}}$} &
        \multicolumn{1}{c||}{$\mathbf{D_{a10}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b4}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b8}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{b9}}$} \\
		\hline
        \hline
        & $|C|$ & 3.8$\cdot$10$^5$ & 1.1$\cdot$10$^6$ & 3.7$\cdot$10$^6$ & 3.9$\cdot$10$^5$ & 2.7$\cdot$10$^7$ & 3.9$\cdot$10$^7$ & 3.1$\cdot$10$^7$ & 4.9$\cdot$10$^7$ & 1.0$\cdot$10$^8$ & - & 11,411 & 1.0$\cdot$10$^6$ & 3.6$\cdot$10$^6$ & 64,398 & 4.9$\cdot$10$^6$ & - \\
        MinHash & $PC$ & 0.910 & 0.987 & 0.903 & 0.903 & 0.903 & 0.985 & 0.936 & 0.948 & 0.923 & - & 0.900 & 0.942 & 0.936 & 0.973 & 0.955 & - \\
        LSH & $PQ$ & 2.6$\cdot$10$^{-4}$ & 0.001 & 2.7$\cdot$10$^{-4}$ & 0.005 & 6.6$\cdot$10$^{-5}$ & 2.7$\cdot$10$^{-5}$ & 3.4$\cdot$10$^{-5}$ & 1.6$\cdot$10$^{-5}$ & 2.1$\cdot$10$^{-5}$ & - & 0.007 & 0.001 & 2.9$\cdot$10$^{-4}$ & 0.036 & 1.7$\cdot$10$^{-5}$ & -\\
        & $RT$ & 212 ms & 717 ms & 4.3 s & 365 ms & 10.3 s & 38.8 s & 12.9 s & 18.3 s & 29.4 s & - & 153 ms & 598 ms & 1.2 s & 2.8 s & 18.8 s & -\\
        \hline
        \hline
        \multirow{4}{*}{\shortstack[c]{Cross-\\ Polytope\\LSH}} & $|C|$ & 23,590 & 1.6$\cdot$10$^5$ & 1.2$\cdot$10$^6$ & 25,344 & 3.2$\cdot$10$^6$ & 4.7$\cdot$10$^6$ & 5.7$\cdot$10$^5$ & 1.9$\cdot$10$^6$ & 9.6$\cdot$10$^6$ & 2.6$\cdot$10$^8$ & 622 & 1.3$\cdot$10$^5$ & 3.5$\cdot$10$^5$ & 2,286	 & 6.9$\cdot$10$^5$ & 1.3$\cdot$10$^6$ \\
        & $PC$ & 0.910 & 0.908 & 0.900 & 0.900 & 0.901 & 0.905 & 0.900 & 0.900 & 0.901 & 0.901 & 	0.910 & 0.911 & 0.902 & 0.901 & 0.917 & 0.908 \\
        & $PQ$ & 0.003 & 0.006 & 0.001 & 0.079 & 0.001 & 2.1$\cdot$10$^{-4}$ & 0.002 & 4.0$\cdot$10$^{-4}$ & 2.2$\cdot$10$^{-4}$	& 7.8$\cdot$10$^{-5}$ & 0.130 & 0.008 & 0.003 & 0.876 & 0.001 & 0.002 \\
        & $RT$ & 181 ms & 902 ms & 4.3 s & 2.0 s & 1.7 s & 1.8 s & 3.6 s & 4.8 s & 19.9 s & 63.9 s & 208 ms & 420 ms & 927 ms & 646 ms & 7.5 s & 7.4 s \\
	    \hline
        \hline
        & $|C|$ & 34,118 & 2.4$\cdot$10$^5$ & 1.8$\cdot$10$^6$ & 34,148 & 4.1$\cdot$10$^6$ & 4.6$\cdot$10$^6$ & 6.7$\cdot$10$^5$ & 3.0$\cdot$10$^6$ & 1.4$\cdot$10$^7$ & 2.8$\cdot$10$^8$ & 1,328 & 1.3$\cdot$10$^5$ & 6.4$\cdot$10$^5$ & 2,375 & 1.9$\cdot$10$^6$ & 87,651 \\
        Hyper- & $PC$ & 0.910 & 0.901 & 0.900 & 0.900 & 0.900 & 0.900 & 0.900 & 0.900 &  
        0.900 & 0.900 & 0.910 & 0.900 & 0.900 & 0.917 & 0.900 & 0.900 \\
        plane LSH & $PQ$ & 0.002 & 0.004 & 0.001 & 0.059 & 4.4$\cdot$10$^{-4}$ & 2.1$\cdot$10$^{-4}$ & 0.001 & 2.6$\cdot$10$^{-4}$ & 1.5$\cdot$10$^{-4}$ & 7.3$\cdot$10$^{-5}$ & 0.061 & 0.007 & 0.002 & 0.859 & 4.0$\cdot$10$^{-4}$ & 0.024 \\
        & $RT$ & 168 ms & 940 ms & 4.2 s & 1.9 s & 1.6 s & 3.5 s & 4.4 s & 7.5 s & 17.5 s & 71.1 s & 246 ms & 430 ms & 930 ms & 943 ms & 5.2 s & 7.0 s \\
        \hline
        \hline
        \multirow{4}{*}{FAISS } & $|C|$ & 1,017 & 30,128 & 1.7$\cdot$10$^6$ & 2,294 & 1.5$\cdot$10$^5$ & 2.0$\cdot$10$^5$ & 24,224 & 5.3$\cdot$10$^5$ & 1.8$\cdot$10$^5$ & 1.3$\cdot$10$^8$8 & 226 & 19,368 & 41,974 & 2,293 & 2.0$\cdot$10$^5$ & 2,516 \\
        & $PC$ & 0.933 & 0.902 & 0.900 & 0.961 & 0.901 & 0.900 & 0.908 & 0.900 & 0.900 & 0.900 & 0.955 & 0.906 & 0.900 & 0.971 & 0.900 & 0.912 \\
        & $PQ$ & 0.082 & 0.032 & 0.001 & 0.932 & 0.012 & 0.005 & 0.041 & 0.001 & 0.012 & 1.5$\cdot$10$^{-4}$ & 0.376 & 0.050 & 0.024 & 0.942 & 0.004 & 0.836 \\
        & $RT$ & 164 ms & 790 ms & 4.2 s & 1.5 s & 1.4 s & 1.8 s & 2.1 s & 7.5 s & 17.7 s & 53.3 s & 204 ms & 264 ms & 787 ms & 901 ms & 5.1 s & 7.4 s \\
        \hline
        \hline
        \multirow{4}{*}{SCANN} & $|C|$ & 1,017 & 30,128 & 1.4$\cdot$10$^6$ & 2,294 & 1.5$\cdot$10$^5$ & 2.0$\cdot$10$^5$ & 24,224 & 4.2$\cdot$10$^5$ & 1.6$\cdot$10$^6$ & 1.3$\cdot$10$^8$ & 226 & 19,368 & 41,974 & 2,293 & 1.5$\cdot$10$^5$ & 2,516 \\
        & $PC$ & 0.933 & 0.902 & 0.900 & 0.961 & 0.901 & 0.900 & 0.908 & 0.900 & 0.900 & 0.900 & 0.966 & 0.906 & 0.900 & 0.970 & 0.900 & 0.912 \\
        & $PQ$ & 0.082 & 0.032 & 0.001 & 0.932 & 0.012 & 0.005 & 0.041 & 0.002 & 0.013 & 1.5$\cdot$10$^{-4}$ & 0.381 & 0.050 & 0.024 & 0.941 & 0.005 & \textbf{\underline{0.836}} \\
        & $RT$ & 182 ms & 828 ms & 4.6 s & 1.8 s & 2.1 s & 2.5 s & 3.0 s & 9.5 s & 29.5 s & 74.4 s & 741 ms & 319	ms & 841 ms & 1.1 s & 9.4 s & 7.8 s \\
        \hline
        \hline
        & $|C|$ & 339 & 37,660 & 5.5$\cdot$10$^5$ & 2,294 & 1.6$\cdot$10$^5$ & 3.2$\cdot$10$^5$ & 7,810 & 43,418 & 10,064 & -
        & 339 & 33,356 & 13,540 & 2,294 & 63,850 & 10,064 \\
        Deep- & $PC$ & 0.943 & 0.903 & 0.900 & 0.983 & 0.901 & 0.900 & 0.926 & 0.900 & 0.908 & - & 0.976 & 0.900 & 0.900 & 0.964 & 0.900 & 0.919 \\
        Blocker & $PQ$ & 0.247 & 0.026 & 0.002 & 0.953 & 0.011 & 0.004 & 0.130 & 0.018 & 0.167 & - & 0.256 & 0.029 & 0.073 & \textbf{\underline{0.953}} & 0.012 & 0.211 \\
        & $RT$ & 6.7 s & 7.5 s & 26.2 s & 18.7 s & 41.4 s & 43.1 s & 46.9 s & 91.1 s & 241.5 s & - & 5.8  s & 5.6	s & 12.2 s & 11.9 s & 89.2 s & 199.8 s \\
        \hline
	\end{tabular}
	\label{tb:nnPerformance}
\end{table*}


==> tables/performance.tex <==
\begin{table*}[t]\centering
\footnotesize
  \setlength{\tabcolsep}{3.6pt}
    \caption{The performance of the fine-tuned blocking workflows across all datasets with respect to number of candidates ($|C|$), recall ($PC$), precision ($PQ$) and overall run-time ($RT$), which is reported in milliseconds ($ms$) or seconds ($s$).}
    \vspace{-10pt}
    \begin{tabular}{ | c l | r  r  r  r  r  r  r  r  r  r || r  r  r  r  r  r  |}
		\cline{3-18}
		\multicolumn{2}{c|}{} &
		\multicolumn{10}{c||}{\textbf{Schema-agnostic}}&
		\multicolumn{6}{c|}{\textbf{Schema-based}}\\
		\multicolumn{2}{c|}{} &
		\multicolumn{1}{c}{$\mathbf{D_{a1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a4}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a5}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a6}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a7}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a8}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a9}}$} &
        \multicolumn{1}{c||}{$\mathbf{D_{a10}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b4}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b8}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{b9}}$} \\
		\hline
        \hline
        \multirow{4}{*}{\shortstack[c]{Standard\\ Blocking\\ (SBW)}} & $|C|$ & 167 & 4,493 & 59,685 & 2,100 & 4,750 & 5,238 & 6,453 & 6,596 & 4,492 & 43,444 & 108 & 3,739 & 4,832 & 2,639 & 27,707 & 3,992 \\
        & $PC$ & 1.000 & 0.902 & 0.901 & 0.903 & 0.922 & 0.924 & 0.909 & 0.904 & 0.915 & 0.904 & 0.933 & 0.901 & 0.922 & 0.976 & 0.904 & 0.906 \\
        & $PQ$ & 0.533 & 0.216 & \underline{0.017} & \textbf{\underline{0.957}} & \textbf{\underline{0.382}} & \textbf{\underline{0.189}} & \underline{0.154} & \underline{0.117} & \underline{0.470} & \textbf{\underline{0.475}} & \textbf{\underline{0.769}} & 0.259 & 0.211 & 0.822 & 0.028 & \underline{0.524} \\
        & $RT$ & 27 ms & 225 ms & 359 ms & 58 ms & 316 ms & 1.1 s & 252 ms & 741 ms & 3.5 s & 57.7 s & 36 ms & 113 ms & 127 ms & 64 ms & 2.7 s & 4.0 s \\
		\hline
		\hline
		\multirow{4}{*}{\shortstack[c]{Q-Grams\\ Blocking\\ (QBW)}} & $|C|$ & 187 & 1,326 & 78,072 & 2,268 & 8,518 & 12,569 & 8,868 & 6,660 & 9,038 & 	59,275 & 110 & 1,312 & 4,217 & 2,704 & 25,819 & 9,231 \\
        & $PC$ & 0.978 & 0.912 & 0.902 & 0.915 & 0.910 & 0.910 & 0.903 & 0.904 & 0.993 & 0.900 & 0.933 & 0.914 & 0.915 & 0.952 & 0.903 & 0.928 \\
        & $PQ$ & 0.465 & 0.740 & 0.013 & 0.897 & 0.210 & 0.078 & 0.112 & 0.116 & 0.254	 & 0.347 & 0.755 & 0.750 & \textbf{\underline{0.240}} & 0.783 & \underline{0.030} & 0.232 \\
        & $RT$ & 46 ms & 75 ms & 340 ms & 92 ms & 234 ms & 1.2 s & 273 ms & 787 ms & 70.0 s & 158.6 s & 21 ms & 38 ms & 237 ms & 45 ms & 6.0 s & 3.6 s \\
        \hline 
        % \multicolumn{17}{c}{\textbf{(c) Extended Q-Grams Blocking Workflow}} \\
        \hline
        \multirow{4}{*}{\shortstack[c]{Extended\\ Q-Grams\\ Blocking\\ (EQBW)}} & $|C|$ & 107 & 4,746 & 81,496 & 2,205 & 8,084 & 12,459 & 7,976 & 8,869 & 14,164 & 52,739 & 110 & 3,719 & 5,307 & 2,377 & 36,076 & 11,530 \\
        & $PC$ & 0.910 & 0.901 & 0.905 & 0.918 & 0.905 & 0.904 & 0.905 & 0.900 & 0.913 & 0.900 & 0.944 & 0.902 & 0.905 & 0.913 & 0.903 & 0.910 \\
        & $PQ$ & 0.757 & 0.204 & 0.012 & 0.926 & 0.220 & 0.078 & 0.124 & 0.087 & 0.149 & 0.390 & 0.764 & 0.261 & 0.188 & \underline{0.854} & 0.021 & 0.182 \\	
        & $RT$ & 303 ms & 347 ms & 2.2 s & 2.6 s & 411 ms & 603 ms & 704 ms & 1.2 s & 6.9 s & 68.1 s & 37 ms	 & 198 ms & 251 ms & 738 ms & 3.9 s & 5.0 s \\
        \hline 
        \hline
        \multirow{4}{*}{\shortstack[c]{Suffix\\ Arrays\\ Blocking\\ (SABW)}} & $|C|$ & 116 & 2,529 & 68,021 & 2,682 & 8,164 & 15,001 & 6,751 & 8,141 & 6,474 & 	1.0$\cdot$10$^6$ & 107 & 2,491 & 4,437 & 3,192 & 79,778 & 1.5$\cdot$10$^5$ \\
        & $PC$ & 1.000 & 0.901 & 0.900 & 0.969 & 0.900 & 0.903 & 0.901 & 0.912 & 0.902	 & 0.900 & 0.910 & 0.903 & 0.909 & 0.997 & 0.900 & 0.877 \\
        & $PQ$ & \textbf{\underline{0.767}} & 0.384 & 0.015 & 0.804 & 0.217 & 0.065 & 0.146 & 0.096 & 0.322 & 	0.020 & 0.757 & 0.390 & 0.226 & 0.695 & 0.010 & 0.014 \\
        & $RT$ & 49 ms & 142 ms & 676 ms & 238 ms & 305 ms & 347 ms & 436 ms & 674 ms & 3.0 s & 9.8 s & 19 ms & 58 ms & 114 ms & 337 ms & 645 ms & 4.5 s \\
        \hline 
        \hline
        Extended & $|C|$ & 175 & 1,277 & 96,064 & 2,674 & 8,819 & 16,473 & 7,261 & 8,705 & 16,016	& 1.5$\cdot$10$^6$ & 109 & 1,243 & 7,567 & 3,683 & 88,236 & 	2.0$\cdot$10$^5$ \\
        Suffix Arrays& $PC$ & 0.921 & 0.901 & 0.902 & 0.902 & 0.900 & 0.900 & 0.901 & 0.900 & 0.900 & 0.901 & 0.910 & 0.901 & 0.901 & 0.902 & 0.900 & 0.865 \\
        Blocking & $PQ$ & 0.469 & \textbf{\underline{0.759}} & 0.010 & 0.751 & 0.201 & 0.059 & 0.136 & 0.088 & 0.130	 & 0.014 & 0.743 & \textbf{\underline{0.780}} & 0.131 & 0.545 & 0.009 & 0.010 \\
        (ESABW) & $RT$ & 161 ms & 281 ms & 891 ms & 745 ms & 388 ms & 481 ms & 750 ms & 1.2 s & 5.6 s & 13.3 s & 23 ms & 187 ms & 418 ms & 201 ms & 1.3 s & 2.2 s \\
        \hline 
        \hline
        \multirow{4}{*}{\shortstack[c]{Parameter-\\ free BW}} & $|C|$ & 290 & 69,340 & 4.6$\cdot$10$^5$ & 1.1$\cdot$10$^5$ & 3.2$\cdot$10$^5$ & 2.6$\cdot$10$^5$ & 4.2$\cdot$10$^5$ & 1.9$\cdot$10$^6$ & 2.3$\cdot$10$^6$ & 6.9$\cdot$10$^7$ & 210 & 6,571 & 6,885 & 2,290 & 38,630 & 3,111 \\
        & $PC$ & 1.000 & 0.981 & 0.971 & 0.999 & 0.998 & 0.995 & 0.991 & 1.000 & 1.000 & 0.980 & 
        0.989 & 0.746 & 0.936 & 0.838 & 0.996 & 0.935 \\
        & $PQ$ & 0.307 & 0.015 & 0.002 & 0.020 & 0.006 & 0.004 & 0.003 & 4.5$\cdot$10$^{-4}$ & 0.001 & 3.3$\cdot$10$^{-4}$ & 0.162 & 0.175 & 0.047 & 0.230 & 5.8$\cdot$10$^{-4}$ & 0.005 \\
        & $RT$ & 29 ms & 32 ms & 135 ms & 44 ms & 76 ms & 81 ms & 125 ms & 243 ms & 579 ms & 5.1 s & 20 ms & 14 ms & 24 ms & 21 ms & 164 ms & 255 ms \\
        \hline
        \hline
        \multirow{4}{*}{\shortstack[f]{Default\\ BW}} & $|C|$ & 3.3$\cdot$10$^5$ & 15,350 & 2.0$\cdot$10$^5$ & 53,203 & 51,573 & 1.2$\cdot$10$^5$ & 1.3$\cdot$10$^5$ & 4.1$\cdot$10$^5$ & 8.4$\cdot$10$^5$ & 2.4$\cdot$10$^6$ & 272 & 5,859 & 14,302 & 35,114 & 1.6$\cdot$10$^5$ & 7.0$\cdot$10$^5$ \\
        & $PC$ & 1.000 & 0.930 & 0.936 & 1.000 & 0.943 & 0.894 & 0.984 & 0.996 & 0.997 & 0.922 & 	0.607 & 0.888 & 0.894 & 0.999 & 0.931 & 0.995 \\
        & $PQ$ & 2.7$\cdot$10$^{-4}$ & 0.065 & 0.005 & 0.042 & 0.036 & 0.008 & 0.008 & 0.002 & 0.003 & 0.009 & 0.199 & 0.163 & 0.069 & 0.063 & 0.005 & 0.003 \\
        & $RT$ & 209 ms & 55 ms & 435 ms & 153 ms & 252 ms & 368 ms & 526 ms & 1.0 s & 2.5 s & 8.2 s & 17 ms & 35 ms & 111 ms & 76 ms & 637 ms & 1.7 s \\
        \hline
	\end{tabular}
	\label{tb:blockingPerformance}
	\vspace{-10pt}
\end{table*}

==> tables/performanceSA.tex <==
\begin{table*}[t]\centering
    \caption{Performance of the fine-tuned filtering methods for the schema-agnostic settings.}
    \vspace{-10pt}
	\begin{tabular}{ | l | l | r | r | r | r | r | r | r | r | r | r |}
		\cline{3-12}
		\multicolumn{2}{c|}{} &
		\multicolumn{1}{c|}{$\mathbf{D_{c1}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c2}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c3}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c4}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c5}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c6}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c7}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c8}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c9}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c10}}$}\\
		\hline
        \hline
        \multirow{ 4}{*}{\textsf{BSL}} & $|C|$ & 290 & 6.9$\cdot$10$^4$ & 4.6$\cdot$10$^5$ & 1.1$\cdot$10$^5$ & 3.2$\cdot$10$^5$ & 2.6$\cdot$10$^5$ & 4.2$\cdot$10$^5$ & 1.9$\cdot$10$^6$ & 2.3$\cdot$10$^6$ & 6.9$\cdot$10$^7$ \\
        & $PC$ & 1.000 & 0.981 & 0.971 & 0.999 & 0.998 & 0.995 & 0.991 & 1.000 & 1.000 & 0.980\\
        & $PQ$ & 0.307 & 0.015 & 0.002 & 0.020 & 0.006 & 0.004 & 0.003 & 4.5$\cdot$10$^4$ & 0.001 & 3.3$\cdot$10$^4$ \\
        &  $RT$ & 29 & 32 & 135 & 44 & 76 & 81 & 125 & 243 & 579 & 5 s \\
        \hline
		\hline
	\end{tabular}
	\label{tb:ccerDatasets}
\end{table*}

==> tables/performanceSB.tex <==
\begin{table*}[t]\centering
    \caption{Performance of the fine-tuned filtering methods for the schema-based settings.}
    \vspace{-10pt}
	\begin{tabular}{ | l | l | r | r | r | r | r | r | r | r | r | r |}
		\cline{3-12}
		\multicolumn{2}{c|}{} &
		\multicolumn{10}{c||}{\textbf{Schema-agnostic}}&
		\multicolumn{10}{c|}{\textbf{Schema-based}}\\
		\multicolumn{2}{c|}{} &
		\multicolumn{1}{c|}{$\mathbf{D_{c1}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c2}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c3}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c4}}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{c5}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c6}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c7}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c8}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c9}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{c10}}$} \\
		\hline
        \hline
        \multirow{ 4}{*}{\textsf{BSL}} & $|C|$ & 543 & 4,593 & 2.2$\cdot$10$^4$ & 8,103 & - & - & - & 1.5$\cdot$10$^6$ & 4.0$\cdot$10$^5$ & - \\
        & $PC$ & 0.989 & 0.746 & 0.936 & 0.838 & - & - & - & 0.996 & 0.935 & - \\
        & $PQ$ & 0.162 & 0.175 & 0.047 & 0.230 & - & - & - & 0.001 & 0.005 & - \\
        &  $RT$ & 20	& 14 & 24 & 21 & 15 & 18 & 15 & 164 & 255 & 140 \\
        \hline
		\hline
	\end{tabular}
	\label{tb:ccerDatasets}
\end{table*}

==> tables/rankingPositions.tex <==
\begin{table*}[t]\centering
% \small
   \setlength{\tabcolsep}{4.5pt}
    \caption{The ranking position of the blocking workflows, the sparse and the dense NN methods with respect to precision.}
    \vspace{-8pt}
    \begin{tabular}{ | l | r  r  r  r  r  r  r  r  r  r | r || r  r  r  r  r  r | r |}
		\cline{2-19}
		\multicolumn{1}{c|}{} &
		\multicolumn{11}{c||}{\textbf{Schema-agnostic Settings}}&
		\multicolumn{7}{c|}{\textbf{Schema-based Settings}}\\
		\multicolumn{1}{c|}{} &
		\multicolumn{1}{c}{$\mathbf{D_{a1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a4}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{a5}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a6}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a7}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a8}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{a9}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{a10}}$} &
        \multicolumn{1}{c||}{Mean} &
        \multicolumn{1}{c}{$\mathbf{D_{b1}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b2}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b3}}$} &
		\multicolumn{1}{c}{$\mathbf{D_{b4}}$} &
        \multicolumn{1}{c}{$\mathbf{D_{b8}}$} &
        \multicolumn{1}{c|}{$\mathbf{D_{b9}}$} &
        \multicolumn{1}{c|}{Mean}  \\
		\hline
        \hline
        SBW & 4 & 5 & 2 & 1 & 1 & 1 & 2 & 2 & 3 & 1 & \textbf{2.2} & 1 & 6 & 4 & 9 & 3 & 5 & 4.7\\
        QBW & 6 & 2 & 4 & 8 & 5 & 3 & 8 & 3 & 5 & 3 & 4.7 & 4 & 2 & 2 & 10 & 2 & 6 & \textbf{4.3} \\
        EQBW & 2 & 6 & 5 & 7 & 3 & 4 & 7 & 6 & 8 & 2 & 5.0 & 2 & 5 & 5 & 7 & 4 & 8 & 5.2 \\
        SABW & 1 & 3 & 3 & 9 & 4 & 5 & 3 & 4 & 4 & 6 & 4.2 & 3 & 3 & 3 & 11 & 7 & 11 & 6.3 \\
        ESABW & 5 & 1 & 6 & 10 & 6 & 6 & 4 & 5 & 9 & 7 & 5.9 & 5 & 1 & 8 & 12 & 8 & 12 & 7.7 \\
        PBW & 7 & 13 & 9 & 16 & 12 & 11 & 14 & 14 & 14 & 9 & 11.9 & 11 & 15 & 11 & 17 & 14  & 14 & 13.7 \\
        DBW & 16 & 9 & 8 & 15 & 7 & 8 & 13 & 11 & 13 & 8 & 10.8 & 17 & 15 & 10 & 15 & 10 & 15 & 13.7 \\
        eJoin & 3 & 8 & 6 & 4 & 8 & 13 & 1 & 7 & 2 & 5 & 5.7 & 6 & 8 & 7 & 4 & 5 & 3 & 5.5 \\
        kNNJ & 9 & 4 & 1 & 2 & 2 & 2 & 6 & 1 & 1 & 4 & 3.2 & 9 & 4 & 1 & 8 & 1 & 4 & 4.5 \\
        DkNN & 12 & 7 & 16 & 11 & 16 & 7 & 12 & 8 & 6 & 14 & 10.9 & 13 & 7 & 6 & 13 & 17 & 9 & 10.8 \\
        MH-LSH & 17 & 16 & 15 & 17 & 15 & 16 & 17 & 17 & 17 & 14 & 16.1 & 16 & 14 & 16 & 16	 & 16 & 17 & 15.8 \\
        CP-LSH & 14 & 14 & 11 & 13 & 13 & 15 & 15 & 15 & 15 & 12 & 13.7 & 12 & 12 & 14 & 5 & 13 & 16 & 12.0 \\
        HP-LSH & 15 & 15 & 13 & 14 & 14 & 14 & 16 & 16 & 16 & 13 & 14.6 & 14 & 13 & 15 & 6 & 15 & 10 & 12.2 \\
        FAISS & 10 & 10 & 14 & 5 & 9 & 9 & 9 & 13 & 11 & 10 & 10.0 & 8 & 9 & 12 & 1 & 12 & 1 & 7.2 \\
        SCANN & 10 & 10 & 12 & 5 & 9 & 9 & 9 & 12 & 10 & 10 & 9.6 & 7 & 9 & 13 & 2 & 11 & 1 & 7.2 \\
        DeepBlocker & 8 & 12 & 9 & 3 & 11 & 12 & 5 & 9 & 7 & 14 & 9.0 & 10 & 11 & 9 & 3 & 6	 & 7 & 7.7 \\
        DDB & 13 & 17 & 16 & 12 & 17 & 17 & 11 & 10 & 12 & 14 & 13.9 & 15 & 15 & 17 & 14 & 9	 & 13 & 13.8 \\
        \hline
        \end{tabular}
	\label{tb:rankingPositions}
	\vspace{-16pt}
\end{table*}


